Patch Validation in Automated Vulnerability Repair

Automated Vulnerability Repair (AVR) systems, especially those leveraging large language models (LLMs), have demonstrated promising results in patching vulnerabilities -- that is, if we trust their patch validation methodology. Ground-truth patches from human developers often come with new tests that not only ensure mitigation of the vulnerability but also encode extra semantics such as root cause location, optimal fix strategy, or subtle coding styles or conventions. And yet, none of the recent AVR systems verify that the auto-generated patches additionally pass these new tests (termed as $\text{PoC}^+$ tests). This is a subtle yet critical omission. To fill this gap, we constructed a benchmark, $\textrm{PVBench}$, with 209 cases spanning 20 projects. Each case includes basic tests (functional tests before the patch and the PoC exploit) as well as the associated $\text{PoC}^+$ tests. Evaluated on three state-of-the-art AVR systems, we find that over 40\% of patches validated as correct by basic tests fail under $\text{PoC}^+$ testing, revealing substantial overestimation on patch success rates. Analyzing these patches that are falsely labeled as correct, we suggest that AVR tools should improve in three critical areas: root cause analysis, adherence to program specifications, and capturing developer intention.

==> Makefile <==
# LaTeX Makefile for main.tex
MAIN = main
LATEX = pdflatex
BIBTEX = bibtex
LATEXFLAGS = -synctex=1 -interaction=nonstopmode -file-line-error

.PHONY: all clean cleanall view

# Default target: full build with bibliography
all: $(MAIN).pdf

# Full build: pdflatex -> bibtex -> pdflatex x2
$(MAIN).pdf: $(MAIN).tex ref.bib sections/*.tex
	$(LATEX) $(LATEXFLAGS) $(MAIN)
	$(BIBTEX) $(MAIN)
	$(LATEX) $(LATEXFLAGS) $(MAIN)
	$(LATEX) $(LATEXFLAGS) $(MAIN)

# Quick build without bibliography
quick:
	$(LATEX) $(LATEXFLAGS) $(MAIN)

# Clean auxiliary files
clean:
	rm -f $(MAIN).aux $(MAIN).bbl $(MAIN).blg $(MAIN).log $(MAIN).out \
	      $(MAIN).toc $(MAIN).lof $(MAIN).lot $(MAIN).fls $(MAIN).fdb_latexmk \
	      $(MAIN).synctex.gz $(MAIN).pyg comment.cut
	rm -f sections/*.aux

# Clean everything including PDF
cleanall: clean
	rm -f $(MAIN).pdf
	rm -rf _minted-$(MAIN)
	rm -f *.pygtex *.pygstyle

# Open PDF (macOS)
view: $(MAIN).pdf
	open $(MAIN).pdf

